Clean Images are Hard to Reblur: Exploiting the Ill-Posed Inverse Task for Dynamic Scene Deblurring

The goal of dynamic scene deblurring is to remove the motion blur in a given image. Typical learning-based approaches implement their solutions by minimizing the L1 or L2 distance between the output and the reference sharp image. Recent attempts adopt visual recognition features in training to improve the perceptual quality. However, those features are primarily designed to capture high-level contexts rather than low-level structures such as blurriness. Instead, we propose a more direct way to make images sharper by exploiting the inverse task of deblurring, namely, reblurring. Reblurring amplifies the remaining blur to rebuild the original blur, however, a well-deblurred clean image with zero-magnitude blur is hard to reblur. Thus, we design two types of reblurring loss functions for better deblurring. The supervised reblurring loss at training stage compares the amplified blur between the deblurred and the sharp images. The self-supervised reblurring loss at inference stage inspects if there noticeable blur remains in the deblurred. Our experimental results on large-scale benchmarks and real images demonstrate the effectiveness of the reblurring losses in improving the perceptual quality of the deblurred images in terms of NIQE and LPIPS scores as well as visual sharpness.

==> sections/figs/srn_lpips_niqe.tex <==
% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=\linewidth]{figs/fig_psnr_lpips/SRN_psnr_lpips.pdf}
%     \end{center}
%     \figcspace
%     \figcspace
%     \caption{
%         \textbf{Test-time adaption results using SRN on GOPRO~\cite{Nah_2017_CVPR} dataset.}
%         The proposed self-supervised objective improves trade-off between the perceptual image quality (LPIPS, NIQE) and PSNR compared with the baseline.
%     }
%     \label{fig:fig_psnr_lpips}
%     \figspace
% \end{figure}



\begin{figure}[t]
    \renewcommand{\wp}{0.50}
    \centering
    \subfloat[PSNR vs LPIPS\label{fig:fig_srn_psnr_lpips}]{\includegraphics[width=\wp\linewidth]{figs_supp/figs_tta/SRN_PSNR_LPIPS.pdf}}
    \hfill
    \subfloat[PSNR vs NIQE\label{fig:fig_srn_psnr_niqe}]{\includegraphics[width=\wp\linewidth]{figs_supp/figs_tta/SRN_PSNR_NIQE.pdf}}
    \figcspace
    \caption{
        \textbf{Test-time adaption results using SRN on GOPRO dataset.}
        The proposed self-supervised objective improves trade-off between the perceptual image quality (LPIPS, NIQE) and PSNR compared with the baseline.
        % \textbf{Perception-distortion trade-off from test-time adaptation applied to SRN model on GOPRO dataset.}
    }
    \label{fig:fig_psnr_lpips}
    \figspace
\end{figure}







==> sections/figs/tta.tex <==
\begin{figure}[t]
    \centering
    \vspace{-3mm}
    \includegraphics[width=\linewidth]{figs/fig_tta/fig_tta_v2.pdf}
    \\
    \figcspace
    \caption{
        \textbf{The proposed self-supervised test-time adaptation.}
        We repetitively find the latent image that reblurs to the current deblurred image.
    }
    \label{fig:fig_tta}
    \figspace
\end{figure}

==> sections/tables/comp_gopro.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabularx}{\linewidth}{p{3cm} | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X }
        \toprule
        Method & LPIPS$_\downarrow$ & NIQE$_\downarrow$ & PSNR$^\uparrow$ & SSIM$^\uparrow$ \\
        \midrule
        U-Net ($\mathcal{L}_{1}$ only) & 0.1635 & 5.996 & 29.66 & 0.8874\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.1365 & 5.629 & 29.58 & 0.8869\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.1238} & \textbf{5.124} & 29.44 & 0.8824\\
        % U-Net ($\mathcal{L}_{1} + \mathcal{L}_{\text{VGG}}$) & 29.43 & 0.8813 & 0.1298 & 5.054\\
        % U-Net ($\mathcal{L}_{1} + 0.01\mathcal{L}_{\text{Adv}}$) &  &  &  & \\
        \midrule
        SRN ($\mathcal{L}_{1}$ only) & 0.1246 & 5.252 & 30.62 & 0.9078\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.1140 & 5.136 & 30.74 & 0.9104\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.1037} & \textbf{4.887} & 30.57 & 0.9074\\
        % SRN ($\mathcal{L}_{1} + \mathcal{L}_{\text{VGG}}$) &  &  &  & \\
        % SRN ($\mathcal{L}_{1} + 0.001\mathcal{L}_{\text{Adv}}$) & 30.53 & 0.9068 & 0.1141 & 4.960\\
        \midrule
        DHN ($\mathcal{L}_{1}$ only) & 0.1179 & 5.490 & 31.53 & 0.9207\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.0975 & 5.472 & 31.53 & 0.9217\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.0837} & \textbf{5.076} & 31.34 & 0.9177\\
        % DHN ($\mathcal{L}_{1} + \mathcal{L}_{\text{VGG}}$) & 31.29 & 0.9167 & 0.0939 & 4.888\\
        % DHN ($\mathcal{L}_{1} + 0.001\mathcal{L}_{\text{Adv}}$) & 31.46 & 0.9188 & 0.0969 & 5.026\\
        \bottomrule
    \end{tabularx}
    \\
    \tabcspace
    \caption{
        \textbf{Perceptual metric improvements from the reblurring loss on GOPRO~\citep{Nah_2017_CVPR} dataset.}
        The reblurring loss consistently improves LPIPS and NIQE over standard $\mathcal{L}_1$ loss.
        % Quantitative comparison on GOPRO~\cite{Nah_2017_CVPR} dataset by reblurring.
    }
    \label{tab:gopro_loss_comparison}
    \tabspace
\end{table}

==> sections/tables/comp_gopro_reds.tex <==
\begin{table}[t]
    \captionsetup{font=footnotesize}
    \footnotesize
    \renewcommand{\arraystretch}{1.15}
    \begin{minipage}[t]{0.49 \linewidth}
        \centering
        \begin{tabularx}{\linewidth}{p{2.15cm} | >{\centering\arraybackslash}X  >{\centering\arraybackslash}X  >{\centering\arraybackslash}X  >{\centering\arraybackslash}X }
            \toprule
            Method & LPIPS$_\downarrow$ & NIQE$_\downarrow$ & PSNR$^\uparrow$ & SSIM$^\uparrow$ \\
            \midrule
            U-Net ($\mathcal{L}_{1}$ only) & 0.1635 & 5.996 & 29.66 & 0.8874\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.1365 & 5.629 & 29.58 & 0.8869\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.1238} & \textbf{5.124} & 29.44 & 0.8824\\
            \midrule
            SRN ($\mathcal{L}_{1}$ only) & 0.1246 & 5.252 & 30.62 & 0.9078\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.1140 & 5.136 & 30.74 & 0.9104\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.1037} & \textbf{4.887} & 30.57 & 0.9074\\
            \midrule
            DHN ($\mathcal{L}_{1}$ only) & 0.1179 & 5.490 & 31.53 & 0.9207\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.0975 & 5.472 & 31.53 & 0.9217\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.0837} & \textbf{5.076} & 31.34 & 0.9177\\
            \bottomrule
        \end{tabularx}
        \tabcspace
        % \caption{
        %     \textbf{Perceptual metric improvements from the reblurring loss on GOPRO~\citep{Nah_2017_CVPR} dataset.}
        %     The reblurring loss consistently improves LPIPS and NIQE over standard $\mathcal{L}_1$ loss.
        %     % Quantitative comparison on GOPRO~\cite{Nah_2017_CVPR} dataset by reblurring.
        % }
        \caption{
        % \textbf{Quantitative comparison on GOPRO~\citep{Nah_2017_CVPR} dataset by loss function.}
        \textbf{Quantitative comparison on GOPRO dataset by loss function.}
        }
        \label{tab:gopro_loss_comparison}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.49 \linewidth}
        \centering
        \begin{tabularx}{\linewidth}{p{2.15cm} | >{\centering\arraybackslash}X  >{\centering\arraybackslash}X  >{\centering\arraybackslash}X  >{\centering\arraybackslash}X }
            \toprule
            Method & LPIPS$_\downarrow$ & NIQE$_\downarrow$ & PSNR$^\uparrow$ & SSIM$^\uparrow$ \\
            \midrule
            U-Net ($\mathcal{L}_{1}$ only) & 0.1486 & 3.649 & 30.80 & 0.8772\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.1435 & 3.487 & 30.76 & 0.8776\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.1252} & \textbf{2.918} & 30.46 & 0.8717\\
            \midrule
            SRN ($\mathcal{L}_{1}$ only) & 0.1148 & 3.392  & 31.89 & 0.8999\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.1071 & 3.305 & 32.01 & 0.9044\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.0947} & \textbf{2.875} & 31.82 & 0.9026\\
            \midrule
            DHN ($\mathcal{L}_{1}$ only) & 0.0942 & 3.288 & 32.65 & 0.9152\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.0931 & 3.248 & 32.57 & 0.9143\\
            \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.0805} & \textbf{2.830} & 32.44 & 0.9122\\
            \bottomrule
        \end{tabularx}
        \tabcspace
        \caption{
        % \textbf{Quantitative comparison on REDS~\citep{Nah_2019_CVPR_Workshops_REDS} dataset by loss function.}
        \textbf{Quantitative comparison on REDS dataset by loss function.}
        % The reblurring loss improves LPIPS and NIQE over standard $\mathcal{L}_1$ loss.
        }
        \label{tab:reds_loss_comparison}
    \end{minipage}
    \tabspace
\end{table}

==> sections/tables/comp_reds.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabularx}{\linewidth}{p{3cm} | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X }
        \toprule
        Method & LPIPS$_\downarrow$ & NIQE$_\downarrow$ & PSNR$^\uparrow$ & SSIM$^\uparrow$ \\
        \midrule
        U-Net ($\mathcal{L}_{1}$ only) & 0.1486 & 3.649 & 30.80 & 0.8772\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.1435 & 3.487 & 30.76 & 0.8776\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.1252} & \textbf{2.918} & 30.46 & 0.8717\\
        \midrule
        SRN ($\mathcal{L}_{1}$ only) & 0.1148 & 3.392  & 31.89 & 0.8999\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.1071 & 3.305 & 32.01 & 0.9044\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.0947} & \textbf{2.875} & 31.82 & 0.9026\\
        \midrule
        DHN ($\mathcal{L}_{1}$ only) & 0.0942 & 3.288 & 32.65 & 0.9152\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n1}}$} & 0.0931 & 3.248 & 32.57 & 0.9143\\
        \multicolumn{1}{r|}{$+ \mathcal{L}_{\text{Reblur, n2}}$} & \textbf{0.0805} & \textbf{2.830} & 32.44 & 0.9122\\
        \bottomrule
    \end{tabularx}
    \\
    \tabcspace
    \caption{
    % Quantitative comparison on REDS~\cite{Nah_2019_CVPR_Workshops_REDS} dataset.
    \textbf{Quantitative comparison on REDS~\citep{Nah_2019_CVPR_Workshops_REDS} dataset by loss function.}
    The reblurring loss improves LPIPS and NIQE over standard $\mathcal{L}_1$ loss.
    }
    \label{tab:reds_loss_comparison}
    \tabspace
\end{table}

==> sections/tables/loss_comp_SRN.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabularx}{\linewidth}{p{3cm} | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X }
        \toprule
        Method & LPIPS$_\downarrow$ & NIQE$_\downarrow$ & PSNR$^\uparrow$ & SSIM$^\uparrow$ \\
        \midrule
        SRN ($\mathcal{L}_{1}$) & 0.1246 & 5.252 & 30.62 & 0.9078\\
        $\qquad \qquad \quad + 0.001\mathcal{L}_{\text{Adv}}$ & 0.1141 & 4.960 & 30.53 & 0.9068\\
        $\qquad \qquad \quad + 0.3\mathcal{L}_{\text{VGG}}$ & \textbf{0.1037} & 4.945 & 30.60 & 0.9074\\
        $\qquad \qquad \quad + \mathcal{L}_{\text{Reblur, n2}}$ & \textbf{0.1037} & \textbf{4.887} & 30.57 & 0.9074\\
        \bottomrule
    \end{tabularx}
    \\
    \tabcspace
    \caption{
        % \textbf{Comparison of reblurring loss and other perceptual losses on GOPRO~\cite{Nah_2017_CVPR} dataset applied to SRN.}
        \textbf{Comparison of reblurring loss and other perceptual losses on GOPRO dataset applied to SRN.}
    }
    \label{tab:comp_reblur_adv}
    \tabspace
\end{table}

==> sections/tables/sharpness_preservation.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabularx}{\linewidth}{p{3cm} | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X }
        \toprule
        Method & LPIPS$_\downarrow$ & NIQE$_\downarrow$ & PSNR$^\uparrow$ & SSIM$^\uparrow$ \\
        \midrule
        U-Net ($\mathcal{L}_\text{Blur}$ only) & 0.1301 & 5.132 & 29.47 & 0.8839\\
        \multicolumn{1}{r |}{$+ \mathcal{L}_\text{Sharp}$ with $S$} & 0.1410 & 5.307 & 29.15 & 0.8694\\
        \multicolumn{1}{r |}{$+ \mathcal{L}_\text{Sharp}$ with $\hat{S}$} & \textbf{0.1238} & \textbf{5.124} & 29.44 & 0.8824\\
        \bottomrule
    \end{tabularx}
    % \tabcspace
    \caption{
        \textbf{The effect of the sharpness preservation in training our reblurring module measured on GOPRO dataset.}
        %
        % In \eqref{eq:eq_loss_sp}, using the pseudo-sharp image $\hat{S}$ instead of the real one $S$ leads to better deblurring performance.
        % %
        % We note that the reblurring module is constructed using 2 ResBlocks.
    }
    \label{tab:gopro_sharpness_preservation}
    \tabspace
\end{table}

==> sections/tables/tta_gopro.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabularx}{\linewidth}{p{3cm} | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X }
        \toprule
        Method & LPIPS$_\downarrow$ & NIQE$_\downarrow$ & PSNR$^\uparrow$ & SSIM$^\uparrow$ \\
        \midrule
        U-Net ($\mathcal{L}_{1}$) & 0.1635 & 5.996 & 29.66 & 0.8874\\
        U-Net ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n1}}$) & 0.1365 & 5.629 & 29.58 & 0.8869\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.1327} & \textbf{5.599} & 29.52 & 0.8878\\
        U-Net ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n2}}$) & 0.1238 & 5.124 & 29.44 & 0.8824\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.1187} & \textbf{5.000} & 29.42 & 0.8831\\
        \midrule
        SRN ($\mathcal{L}_{1}$) & 0.1246 & 5.252 & 30.62 & 0.9078\\
        %\midrule
        SRN ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n1}}$) & 0.1140 & 5.136 & 30.74 & 0.9104\\
        % \multicolumn{1}{r |}{$+$ TTA step 1} & 0.1129 & 5.125 & 30.74 & 0.9107\\
        % % \multicolumn{1}{r |}{$+$ TTA step 2} & 0.1119 & 5.113 & 30.73 & 0.9108\\
        % \multicolumn{1}{r |}{$+$ TTA step 3} & 0.1112 & 5.101 & 30.70 & 0.9108\\
        % % \multicolumn{1}{r |}{$+$ TTA step 4} & 0.1105 & 5.090 & 30.66 & 0.9105\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.1101} & \textbf{5.079} & 30.60 & 0.9100\\
        %\midrule
        SRN ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n2}}$) & 0.1037 & 4.887 & 30.57 & 0.9074\\
        % + TTA step 1 & 0.1024 & 4.858 & 30.56 & 0.9075\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.0983} & \textbf{4.730} & 30.44 & 0.9067\\
        \midrule
        DHN ($\mathcal{L}_{1}$) & 0.1179 & 5.490 & 31.53 & 0.9207\\
        %\midrule
        DHN ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n1}}$) & 0.0975 & 5.472 & 31.53 & 0.9217\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.0940} & \textbf{5.343} & 31.32 & 0.9208\\
        %\midrule
        DHN ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n2}}$) & 0.0837 & 5.076 & 31.34 & 0.9177\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.0805} & \textbf{4.948} & 31.28 & 0.9174\\
        \bottomrule
    \end{tabularx}
    \\
    \tabcspace
    \caption{
        \textbf{Test-time adaptation results of various deblurring networks on GOPRO dataset.}
    }
    \label{tab:gopro_tta_comparison}
    \tabspace
\end{table}

==> sections/tables/tta_reds.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabularx}{\linewidth}{p{3cm} | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X }
        \toprule
        Method & LPIPS$_\downarrow$ & NIQE$_\downarrow$ & PSNR$^\uparrow$ & SSIM$^\uparrow$ \\
        \midrule
        U-Net ($\mathcal{L}_{1}$) & 0.1486 & 3.649 & 30.80 & 0.8772\\
        U-Net ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n1}}$) & 0.1435 & 3.487 & 30.76 & 0.8776\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.1403} & \textbf{3.476} & 30.64 & 0.8781\\
        U-Net ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n2}}$) & 0.1252 & 2.918 & 30.46 & 0.8717\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.1226} & \textbf{2.849} & 30.25 & 0.8701\\
        \midrule
        SRN ($\mathcal{L}_{1}$) & 0.1148 & 3.392 & 31.89 & 0.8999\\
        SRN ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n1}}$) & 0.1071 & 3.305 & 32.01 & 0.9044\\
        % + TTA step 1 & 0.1060 & 3.297 & 32.01 & 0.9047\\
        % + TTA step 2 & 0.1050 & 3.292 & 31.99 & 0.9048\\
        % + TTA step 3 & 0.1042 & 3.286 & 31.95 & 0.9047\\
        % + TTA step 4 & 0.1035 & 3.282 & 31.90 & 0.9045\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.1029} & \textbf{3.278} & 31.83 & 0.9040\\
        SRN ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n2}}$) & 0.0947 & 2.875 & 31.82 & 0.9026\\
        % + TTA step 1 & 0.0936 & 2.858 & 31.78 & 0.9026\\
        % + TTA step 2 & 0.0927 & 2.842 & 31.74 & 0.9024\\
        % + TTA step 3 & 0.0919 & 2.827 & 31.67 & 0.9021\\
        % + TTA step 4 & 0.0913 & 2.812 & 31.59 & 0.9015\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.0909} & \textbf{2.798} & 31.50 & 0.9008\\
        \midrule
        DHN ($\mathcal{L}_{1}$) & 0.0942 & 3.288 & 32.65 & 0.9152\\
        %\midrule
        %DHN ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n1}}$) & 0.0931 & 3.248 & 32.57 & 0.9143\\
        %+ TTA step 5 & \textbf{0.0887} & \textbf{3.220} & 32.38 & 0.9139\\
        %\midrule
        DHN ($\mathcal{L}_{1} + \mathcal{L}_{\text{Reblur, n2}}$) & 0.0805 & 2.830 & 32.44 & 0.9122\\
        \multicolumn{1}{r |}{$+$ TTA step 5} & \textbf{0.0763} & \textbf{2.761} & 32.17 & 0.9110\\
        \bottomrule
    \end{tabularx}
    \tabcspace
    \caption{
        \textbf{Test-time adaptation results of various deblurring methods on REDS dataset.}
    }
    \label{tab:reds_tta_comparison}
    \tabspace
\end{table}
